Abstraction-Guided Truncations for Stationary Distributions of Markov Population Models

To understand the long-run behavior of Markov population models, the computation of the stationary distribution is often a crucial part. We propose a truncation-based approximation that employs a state-space lumping scheme, aggregating states in a grid structure. The resulting approximate stationary distribution is used to iteratively refine relevant and truncate irrelevant parts of the state-space. This way, the algorithm learns a well-justified finite-state projection tailored to the stationary behavior. We demonstrate the method's applicability to a wide range of non-linear problems with complex stationary behaviors.

==> splitting_fig.tex <==
    \begin{minipage}{.3\textwidth}
    \begin{tikzpicture}
    \tikzstyle{vertex}=[circle,minimum size=5mm,draw,text=black]
\node[vertex]
    (N1) at (-1.5,.75)
    { };
\node[vertex,fill=black!25]
    (N2) at (0, 0)
    { };
\node[vertex]
    (N3) at (1.5, 0)
    { };
\node[vertex]
    (N4) at (-1.5, -.75)
    { };
\node[vertex]
    (N5) at (1, 1)
    { };

\draw[->,line width=.8pt] (N5) to [bend left=10] (N3);
\draw[->,line width=.8pt] (N3) to [bend left=10] (N5);

\draw[->,line width=.8pt] (N1) to[bend left=10] (N2);
\draw[->,line width=.8pt] (N2) to[]             (N3);
\draw[->,line width=.8pt] (N2) to[bend left=10] (N4);

\draw[densely dashed, line width=1pt] (-.5, -1) -- (.5, 1);
\end{tikzpicture}
 \end{minipage}
 \hfill
 \begin{minipage}{.3\textwidth}
    \begin{tikzpicture}
\tikzstyle{vertex}=[circle,minimum size=5mm,draw,text=black]
\node[vertex]
    (N1) at (-1.5,.75)
    { };
\node[vertex,fill=black!25]
    (N2a) at (-.5, 0)
    { };
\node[vertex,fill=black!25]
    (N2b) at (.5, 0)
    { };
\node[vertex]
    (N3) at (1.5, 0)
    { };
\node[vertex]
    (N4) at (-1.5, -.75)
    { };
\node[vertex]
    (N5) at (1, 1)
    { };
\node[circle,minimum size=5mm,draw,text=black]
    (N1) at (-1.5,.75)
    { };


\draw[->,line width=.8pt] (N5) to [bend left=10] (N3);
\draw[->,line width=.8pt] (N3) to [bend left=10] (N5);

\draw[->,dashed,line width=.8pt] (N1)  to[bend left=10]  (N2a);
\draw[->,dashed,line width=.8pt] (N2a) to[bend right=40] (N3);
\draw[->,dashed,line width=.8pt] (N2a) to[bend left=10]  (N4);

\draw[->,dashed,line width=.8pt] (N1)  to[bend left=10] (N2b);
\draw[->,dashed,line width=.8pt] (N2b) to[]             (N3);
\draw[->,dashed,line width=.8pt] (N2b) to[bend left=10] (N4);

\draw[->,dashed,line width=.8pt] (N2a) to [bend left=10] (N2b);
\draw[->,dashed,line width=.8pt] (N2b) to [bend left=10] (N2a);
\end{tikzpicture}
    \end{minipage}
     \hfill
 \begin{minipage}{.3\textwidth}
    \begin{tikzpicture}
\tikzstyle{vertex}=[circle,minimum size=5mm,draw,text=black]
\node[vertex]
    (N1) at (-1.5,.75)
    { };
\node[vertex,fill=black!25]
    (N2a) at (-.5, 0)
    { };
\node[vertex,fill=black!25]
    (N2b) at (.5, 0)
    { };
\node[vertex]
    (N3) at (1.5, 0)
    { };
\node[vertex]
    (N4) at (-1.5, -.75)
    { };
\node[vertex]
    (N5) at (1, 1)
    { };
\node[circle,minimum size=5mm,draw,text=black]
    (N1) at (-1.5,.75)
    { };

\draw[->,line width=.8pt] (N5) to [bend left=10] (N3);
\draw[->,line width=.8pt] (N3) to [bend left=10] (N5);

\draw[->,line width=.8pt] (N1)  to[bend left=10]  (N2a);
\draw[->,line width=.8pt] (N2a) to[bend left=10]  (N4);

\draw[->,line width=.8pt] (N1)  to[bend left=10] (N2b);
\draw[->,line width=.8pt] (N2b) to[]             (N3);

\draw[->,line width=.8pt] (N2b) to [bend left=10] (N2a);
\end{tikzpicture}
    \end{minipage}
